Updated Combination of Searches for the Standard Model Higgs Boson at the D0 Experiment in 9.7 fb-1 of Data

Searches for standard model Higgs boson production at the D0 experiment in ppbar collisions at sqrt(s)=1.96 TeV are carried out for Higgs boson masses (m_H) in the range 100<m_H<200 GeV. Most of these searches use the full Run II data set, corresponding to an integrated luminosity of 9.7 fb-1, and are combined to maximize the sensitivity to the standard model Higgs boson. In absence of a significant excess above the background expectation, 95% confidence level upper limits are set on the production cross section for a standard model Higgs boson. The upper limits are found to be a factor of 2.11 (0.73) times the predicted standard model cross section for m_H=115 (165) GeV. Under the background-only hypothesis, the corresponding expected limit is 1.46 (0.72) times the standard model prediction. At the same confidence level, these analyses exclude a standard model Higgs boson with a mass in the range 159<m_H<170 GeV, while the a priori expected exclusion is 156<mH<173 GeV. In the range 120<mH<140 GeV, the data exhibit an excess over the background prediction of approximately two Gaussian standard deviations.

==> d0-sys-tautaujj-eps2011.tex <==
\begin{table}[hp]
\begin{center}
\caption{\label{tab:d0sysVHtau}  Systematic uncertainties on the signal and background contributions for
D0's
%$XH\rightarrow \ell \tau$jj Run~IIb channel ($l=e,\mu$).
$\tau \tau jj$ Run~IIb channel.
Systematic uncertainties for the
Higgs signal shown in this table are obtained for $m_H=135$ GeV/$c^2$.  Systematic uncertainties are listed
by name; see the original references for a detailed explanation of their meaning and on how they are derived.
Uncertainties are relative, in percent, and are symmetric unless otherwise indicated. A systematic is denoted
as flat if it affects the normalization only, and as a shape ``S'' uncertainty otherwise.}
\vskip 0.1cm
%{\centerline{D0: $XH\rightarrow \mu \tau_{\rm{had}} jj$ Run~IIb channel relative uncertainties (\%)}}
{\centerline{D0: $\mu \tau_{\rm{had}} jj$ Run IIb channel relative uncertainties (\%)}}
\vskip 0.099cm
\begin{ruledtabular}
\begin{tabular}{lccccccccc}\\
Contribution &$VH$ Signal &$VBF$ Signal &$ggH$ Signal  &$W+jets$ & $Z+jets$ & Top& diboson& Multijet\\ \hline


Luminosity (D0 specific)  & 4.1 & 4.1 & 4.1 & 4.1 & 4.1 & 4.1 &4.1 &- \\
Luminosity (Tevatron common)  & 4.6 & 4.6 & 4.6 & 4.6 & 4.6 & 4.6 &4.6 &- \\
$\mu$ ID & 2.9 & 2.9 & 2.9 & 2.9 & 2.9 & 2.9 &2.9 &- \\
$\mu$ trigger & 8.6 & 8.6 & 8.6 & 8.6 & 8.6 & 8.6 &8.6 &- \\
$\tau$ energy correction & 9.8 & 9.8 & 9.8 & 9.8 & 9.8 & 9.8 &9.8 &- \\
$\tau$ track efficiency & 1.4 & 1.4 & 1.4 & 1.4 & 1.4 & 1.4 &1.4 &- \\
$\tau$ selection by type & 12,4.2,7 & 12,4.2,7 & 12,4.2,7 & 12,4.2,7 & 12,4.2,7 & 12,4.2,7 &12,4.2,7 &- \\
Cross section & 6.2 &4.9& 33 &6.0&6.0&10.0&7.0&-\\
ggH Signal PDF &-&-&29&-&-&-&-&-\\
ggH $H p_T$ Reweighting (S)& 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 &1.0 &-\\
Signal Branching Fraction & 0-7.3 & 0-7.3 & 0-7.3 & - & - & - & - &-\\
Vertex confirmation for jets  & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 &4.0 &- \\


Jet ID(S)  & $\sim$10 & $\sim$10 & $\sim$10 & $\sim$10& $\sim$10 & $\sim$10 &$\sim$10 &- \\
Jet Energy Resolution (S)  & $\sim$10 & $\sim$10 & $\sim$10 & $\sim$10& $\sim$10 & $\sim$10 &$\sim$10 &- \\
Jet energy Scale (S)  & $\sim$15 & $\sim$15 & $\sim$15 & $\sim$15& $\sim$15 & $\sim$15 &$\sim$15 &- \\


Jet pT  & 5.5 & 5.5 & 5.5 & 5.5 & 5.5 & 5.5 &5.5 &- \\
PDF reweighting  & 2 & 2 & 2 & 2 & 2 & 2 &2 &- \\
Multijet Normalization  & - & - & - & - & - & - &- &5.3 \\
Multijet Shape   & - & - & - & - & - & - &- &$\sim$15 \\

\end{tabular}
\end{ruledtabular}


\vskip 0.3cm
%{\centerline{D0: $XH\rightarrow e \tau_{\rm{had}} jj$ Run~IIb relative uncertainties (\%)}}
{\centerline{D0: $e \tau_{\rm{had}} jj$ Run IIb relative uncertainties (\%)}}
\vskip 0.099cm
\begin{ruledtabular}
\begin{tabular}{lccccccccc}\\
Contribution &$VH$ Signal &$VBF$ Signal &$ggH$ Signal  &$W+jets$ & $Z+jets$ & Top& diboson& Multijet\\
\hline
Luminosity (D0 specific)  & 4.1 & 4.1 & 4.1 & 4.1 & 4.1 & 4.1 &4.1 &- \\
Luminosity (Tevatron common)  & 4.6 & 4.6 & 4.6 & 4.6 & 4.6 & 4.6 &4.6 &- \\
EM ID & 4 & 4 & 4 & 4 & 4 & 4 &4 &- \\
e trigger & 2 & 2 & 2 & 2 & 2 & 2 &2 &- \\
$\tau$ energy correction & 9.8 & 9.8 & 9.8 & 9.8 & 9.8 & 9.8 &9.8 &- \\
$\tau$ track efficiency & 1.4 & 1.4 & 1.4 & 1.4 & 1.4 & 1.4 &1.4 &- \\
$\tau$ selection by type & 12,4.2,7 & 12,4.2,7 & 12,4.2,7 & 12,4.2,7 & 12,4.2,7 & 12,4.2,7 &12,4.2,7 &- \\
Cross section & 6.2 &4.9& 33 &6.0&6.0&10.0&7.0&-\\
ggH Signal PDF &-&-&29&-&-&-&-&-\\
ggH $H p_T$ Reweighting (S)& 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 &1.0 &-\\
Signal Branching Fraction & 0-7.3 & 0-7.3 & 0-7.3 & - & - & - & - &-\\
Vertex confirmation for jets  & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 &4.0 &- \\

Jet ID(S)  & $\sim$10 & $\sim$10 & $\sim$10 & $\sim$10& $\sim$10 & $\sim$10 &$\sim$10 &- \\
Jet Energy Resolution (S)  & $\sim$10 & $\sim$10 & $\sim$10 & $\sim$10& $\sim$10 & $\sim$10 &$\sim$10 &- \\
Jet energy Scale (S)  & $\sim$15 & $\sim$15 & $\sim$15 & $\sim$15& $\sim$15 & $\sim$15 &$\sim$15 &- \\

Jet pT  & 5.5 & 5.5 & 5.5 & 5.5 & 5.5 & 5.5 &5.5 &- \\
PDF reweighting  & 2 & 2 & 2 & 2 & 2 & 2 &2 &- \\
Multijet Normalization  & - & - & - & - & - & - &- &4.7 \\
Multijet Shape   & - & - & - & - & - & - &- & $\sim$15 \\


\end{tabular}
\end{ruledtabular}

\end{center}
\end{table}


==> d0-sys-tautaujj-m2012.tex <==
\begin{table}[hp]
\begin{center}
\caption{\label{tab:d0sysVHtau}  Systematic uncertainties on the signal and background contributions for 
D0's
%$XH\rightarrow l \tau$jj Run~IIb channel ($l=e,\mu$). 
$\tau \tau jj$ Run IIb channel. 
Systematic uncertainties for the 
Higgs signal shown in this table are obtained for $m_H=135$ GeV/$c^2$.  Systematic uncertainties are listed 
by name; see the original references for a detailed explanation of their meaning and on how they are derived.  
Uncertainties are relative, in percent, and are symmetric unless otherwise indicated. Shape
      uncertainties are labeled with an ``(S).''}
\vskip 0.1cm
%{\centerline{D0: $XH\rightarrow \mu \tau_{had} jj$ Run IIb channel relative uncertainties (\%)}}
{\centerline{$\mu \tau_{had} jj$ Run~IIb channel relative uncertainties (\%)}}
\vskip 0.099cm
\begin{ruledtabular}
\begin{tabular}{lccccccccc}\\
%Contribution &$VH$  &\pvbf & $gg\to H$  &$W$+jets & $Z$+jets & Top& Dibosons& Multijet\\ \hline
Contribution &$VH$  &$VBF$& $ggH$  &$W$+jets & $Z$+jets & Top& Dibosons& Multijet\\ \hline

Luminosity   & 6.1 & 6.1 & 6.1 & 6.1 & 6.1 & 6.1 &6.1 &-- \\ 
$\mu$ ID & 2.9 & 2.9 & 2.9 & 2.9 & 2.9 & 2.9 &2.9 &-- \\ 
$Single \mu$ trigger & 5.0 & 5.0 & 5.0 & 5.0 & 5.0 & 5.0 &5.0 &-- \\ 
inclusive trigger relative & 7.0 & 7.0 & 7.0 & 7.0 & 7.0 & 7.0 &7.0 &-- \\ 
$\tau$ energy correction & 9.8 & 9.8 & 9.8 & 9.8 & 9.8 & 9.8 &9.8 &-- \\ 
$\tau$ track efficiency & 1.4 & 1.4 & 1.4 & 1.4 & 1.4 & 1.4 &1.4 &-- \\ 
$\tau$ selection by type & 10,4,5 & 10,4,5 & 10,4,5 & 10,4,5 & 10,4,5 & 10,4,5 &10,4,5 &-- \\ 
Cross section & 6.2 &4.9& 33 &6.0&6.0&10.0&7.0&--\\
GGF Signal PDF &--&--&29&--&--&--&--&--\\
GGF $H p_T$ Reweighting (S)& -- & -- $\sim$5.0 & -- &  -- &  -- & -- &-- &--\\
Signal Branching Fraction  & 0-7.3 & 0-7.3  & 0-7.3 &  -- &  -- &  -- &  -- &  --\\
Vertex confirmation for jets(S)  & $\sim$ 5.0 &  $\sim$5.0 &  $\sim$5.0 &  $\sim$5.0 &  $\sim$5.0 &  $\sim$5.0 & $\sim$5.0 &-- \\ 


Jet ID(S)  & $\sim$5 & $\sim$5 & $\sim$5 & $\sim$5& $\sim$5 & $\sim$5 &$\sim$5 &-- \\
Jet Energy Resolution (S)  & $\sim$5 & $\sim$5 & $\sim$5 & $\sim$5& $\sim$5 & $\sim$5 &$\sim$5 &-- \\
Jet energy Scale (S)  & $\sim$5 & $\sim$5 & $\sim$5 & $\sim$5& $\sim$5 & $\sim$5 &$\sim$5 &-- \\


Jet pT  & 5.5 & 5.5 & 5.5 & 5.5 & 5.5 & 5.5 &5.5 &-- \\
PDF reweighting   & 1.6 & 1.6 & 1.6 & 1.6 & 2 & 2 &2 &-- \\
Multijet Normalization  & -- & -- & -- & -- & -- & -- &-- &5.3 \\
Multijet Shape   & -- & -- & -- & -- & -- & -- &-- &$\sim$15 \\

\end{tabular}
\end{ruledtabular}


\vskip 0.3cm
%{\centerline{D0: $XH\rightarrow e \tau_{had} jj$ Run IIb relative uncertainties (\%)}}
{\centerline{$e \tau_{had} jj$ Run~IIb relative uncertainties (\%)}}
\vskip 0.099cm
\begin{ruledtabular}
\begin{tabular}{lccccccccc}\\
%Contribution &$VH$  &\pvbf & $gg\to H$  &$W$+jets & $Z$+jets & Top& Dibosons& Multijet\\ 
Contribution &$VH$  &$VBF$& $ggH$  &$W$+jets & $Z$+jets & Top& Dibosons& Multijet\\ \hline
\hline
Luminosity  & 6.1 & 6.1 & 6.1 & 6.1 & 6.1 & 6.1 &6.1 &-- \\ 
Electron ID & 4 & 4 & 4 & 4 & 4 & 4 &4 &-- \\ 
Electron trigger & 2 & 2 & 2 & 2 & 2 & 2 &2 &-- \\ 
$\tau$ energy correction & 9.8 & 9.8 & 9.8 & 9.8 & 9.8 & 9.8 &9.8 &-- \\ 
$\tau$ track efficiency & 1.4 & 1.4 & 1.4 & 1.4 & 1.4 & 1.4 &1.4 &-- \\ 
$\tau$ selection by type & 10,4,5 & 10,4,5 & 10,4,5 & 10,4,5 & 10,4,5 & 10,4,5 &10,4,5 &-- \\ 
Cross section & 6.1 &4.9& 33 &6.0&6.0&10.0&7.0&--\\
GGF Signal PDF &--&--&29&--&--&--&--&--\\
GGF $H p_T$ Reweighting (S)& -- & -- & $\sim$ 5.0 & -- & -- & -- &-- &--\\
Signal Branching Fraction  & 0-7.3 & 0-7.3  & 0-7.3 &  -- &  -- &  -- &  -- &  --\\
Vertex confirmation for jets(S)  & $\sim$ 5.0 &  $\sim$5.0 &  $\sim$5.0 &  $\sim$5.0 &  $\sim$5.0 &  $\sim$5.0 & $\sim$5.0 &-- \\ 

Jet ID(S)  & $\sim$10 & $\sim$5 & $\sim$5 & $\sim$5& $\sim$5 & $\sim$5 &$\sim$5 &-- \\
Jet Energy Resolution (S)  & $\sim$10 & $\sim$10 & $\sim$10 & $\sim$10& $\sim$10 & $\sim$10 &$\sim$10 &-- \\
Jet energy Scale (S)  & $\sim$10 & $\sim$10 & $\sim$10 & $\sim$10& $\sim$10 & $\sim$10 &$\sim$10 &-- \\

Jet pT  & 5.5 & 5.5 & 5.5 & 5.5 & 5.5 & 5.5 &5.5 &-- \\
PDF reweighting  & 1.6 & 1.6 & 1.6 & 1.6 & 2 & 2 &2 &-- \\
Multijet Normalization  & -- & -- & -- & -- & -- & -- &-- &4.7 \\
Multijet Shape   & -- & -- & -- & -- & -- & -- &-- & $\sim$15 \\


\end{tabular}
\end{ruledtabular}

\end{center}
\end{table}


==> d0-sys-ttl-m2012.tex <==
%\def\D0{D\O }
\begin{table}[hp]
\begin{center}
\caption{\label{tab:d0systwwlvlv} 
Systematic uncertainties on the signal and background contributions
for D0's $\tau\tau\mu$ +X 
channel.  Systematic uncertainties are listed by name; see the
original references for a detailed explanation of their meaning and on
how they are derived.  Shape uncertainties are labeled with the ``s''
designation. Cross section uncertainties on
the $gg\to H$ signal depend on the jet multiplicity, as described in
the main text. Uncertainties are relative, in percent, and are
symmetric unless otherwise indicated.
}\vskip 0.1cm
%{\centerline{{$\tau\tau\mu$ +X  channel relative uncertainties (\%)}}
{\centerline{$\tau\tau\mu$ +X  channels relative uncertainties (\%)}}
\vskip 0.099cm
\begin{ruledtabular}
\begin{tabular}{ l  c  c  c  c  c  c  c  c  }  \\
Contribution & Dibosons & ~~$Z/\gamma^*$~~&~~~~$t\bar{t}~~~~$    & ~~Instrumental~~  & $gg\to H$ & $qq\to qqH$ & $VH$ \\ 
\hline
Luminosity/Normalization    &  6      &   6                     & 6            &  24   &   6  &   6  &   6  \\
Trigger &  3      &   3                     & 3           & --   &   3  &   3  &   3  \\
Cross Section (Scale/PDF)      &  7        &   6           & 10                       &  --  &   13-33/7.6-30 & 4.9 & 6.2  \\
PDF              &      2.5     &   2.5          & 2.5                 &  --   &   2.5   &   2.5     &   2.5      \\
Tau Id per $\tau$  (Type 1/2/3)    &  7/3.5/5  &   7/3.5/5                   & 7/3.5/5      &  --   &   7/3.5/5       &   7/3.5/5        &   7/3.5/5         \\
Tau Energy Scale &  1  &   1                  & 1    &  --   &   1     &   1        &  1      \\
Tau Track Match per $\tau$&  1.4  &   1.4                  & 1.4    &  --   &   1.4     &   1.4        &  1.4      \\
Muon Identification     &  2.9           &  2.9                       & 2.9            &  --   &   2.9      &   2.9     &   2.9       \\
\end{tabular}
\end{ruledtabular}
\end{center}
\end{table}





==> needspace/README <==

The NEEDSPACE package
=====================

Provides the \needspace and \Needspace macros for
requesting a certain amount of space on the current
page for the following material.


INSTALLATION
------------

Run `pdflatex` on needspace.tex to produce the files
  needspace.ins and needspace.sty,
as well as to compile the PDF documentation.

Execute `tex needspace.ins` to produce the files above
except needspace.ins itself (and the PDF file, obviously).


CHANGE HISTORY
--------------

* v1.3c (2010/09/12):  
  Patch to improve behaviour with commands like `\section` that use
  `\addvspace`. See [this thread][ctt] on comp.text.tex.

[ctt]: http://groups.google.com/group/comp.text.tex/browse_frm/thread/8d849a1e0be2120e

* v1.3b (2009/09/03):  
  New maintainer (Will Robertson)

* v1.3a (2003/02/18):  
  At the suggestion of Donald Arseneau (private emails) changed guts of
  \needspace from
  
        ... \vskip\z@\@plus\dimen@\pagebreak[3]\vskip\z@\@plus-\dimen@\endgroup}

* v1.3 (2003/02/07):  
  Added \Needspace (an extended version of postings by Donald Arseneau 
  to comp.text.tex e.g., in November 1993, August 1995, September 1997, ...)

* v1.2 (2002/09/11):  
  At the suggestion of Robin Fairbairns, added use of \dimen@ to capture 
  the argument so that calc package commands can be used in the argument.


COPYRIGHT AND LICENSING
-----------------------

Authors: Donald Arseneau and Peter Wilson (Herries Press)  
Maintainer: Will Robertson (will dot robertson at latex-project dot org)  
Copyright 1996-2003 Peter Wilson  
Copyright 2010 Will Robertson  

This work may be distributed and/or modified under the
conditions of the LaTeX Project Public License, either
version 1.3c of this license or (at your option) any
later version: <http://www.latex-project.org/lppl.txt>

This work has the LPPL maintenance status "maintained".
The Current Maintainer of this work is Will Robertson.

This work consists of the files needspace.tex and the
derived files needspace.sty and needspace.ins.


MAINTENANCE
-----------

Please report bugs or request features:  
  <http://github.com/wspr/herries-press/issues>

Developmental and historical versions:  
  <http://github.com/wspr/herries-press>

Current release version:   
  <http://ctan.tug.org/pkg/needspace>  


